Deep-Bench: Deep Learning Benchmark Dataset for Code Generation

Deep learning (DL) has revolutionized areas such as computer vision, natural language processing, and more. However, developing DL systems is challenging due to the complexity of DL workflows. Large Language Models (LLMs), such as GPT, Claude, Llama, Mistral, etc., have emerged as promising tools to assist in DL code generation, offering potential solutions to these challenges. Despite this, existing benchmarks such as DS-1000 are limited, as they primarily focus on small DL code snippets related to pre/post-processing tasks and lack a comprehensive coverage of the full DL pipeline, including different DL phases and input data types. To address this, we introduce DeepBench, a novel benchmark dataset designed for function-level DL code generation. DeepBench categorizes DL problems based on three key aspects: phases such as pre-processing, model construction, and training; tasks, including classification, regression, and recommendation; and input data types such as tabular, image, and text. GPT-4o -- the state-of-the-art LLM -- achieved 31% accuracy on DeepBench, significantly lower than its 60% on DS-1000. We observed similar difficulty for other LLMs (e.g., 28% vs. 54% for Claude, 21% vs. 41% for LLaMA, and 15% vs. 20% for Mistral). This result underscores DeepBench's greater complexity. We also construct a taxonomy of issues and bugs found in LLM-generated DL code, which highlights the distinct challenges that LLMs face when generating DL code compared to general code. Furthermore, our analysis also reveals substantial performance variations across categories, with differences of up to 7% among phases and 37% among tasks. These disparities suggest that DeepBench offers valuable insights into the LLMs' performance and areas for potential improvement in the DL domain.

==> figs/accepted1.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/box_x.pdf}
    %\vspace{-7pt}
    \caption{Pre/post processing example: Converting formats of bounding boxes
    }
    \label{fig:accepted1}
    %\vspace{-10pt}
\end{figure}

==> figs/accepted2.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{pics/Accepted2.pdf}
    \vspace{-7pt}
    \caption{Another example of data GPT is able to generate the code
    }
    \label{fig:accepted2}
    \vspace{-10pt}
\end{figure}

==> figs/accepted_table.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figs/adapted_c.pdf}
    %\vspace{-7pt}
    \caption{Structured Array example: Generating function to compute adapted Cohen Kappa score based on an array}
    \label{fig:accepted_structured}
    %\vspace{-10pt}
\end{figure}

==> figs/accs.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{pics/stepsacc.png}
    \vspace{-7pt}
    \caption{Accuracy based on different categories
    }
    \label{fig:accs_steps}
    \vspace{-10pt}
\end{figure*}

==> figs/accs_datatype.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{pics/dataaccs.png}
    \vspace{-7pt}
    \caption{Accuracy based on different data types
    }
    \label{fig:accs_datatypes}
    \vspace{-10pt}
\end{figure*}

==> figs/accs_tasks.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{pics/taskaccs.png}
    \vspace{-7pt}
    \caption{Accuracy based on different data types
    }
    \label{fig:accs_tasks}
    \vspace{-10pt}
\end{figure*}

==> figs/accs_v2.tex <==
\begin{figure}[t!]
\pgfplotsset{compat=1.18}

\begin{tikzpicture}
\begin{groupplot}[
    group style={
        group name=my plots, 
        group size=3 by 2, 
        xlabels at=edge bottom, 
        ylabels at=edge left,
        vertical sep = 1.5cm
    },
    height=0.33\linewidth, 
    width=0.36\linewidth, 
    ylabel={Correct Instances},
    ybar, 
    enlargelimits=0.15, 
    symbolic x coords={A, B, C, D, E, F, G, H, I}, 
    xtick=\empty,
    % xticklabels = {}
    legend style={
        at={(1.7,1.35)}, 
        anchor=south, 
        legend columns=5, 
        /tikz/every even column/.append style={column sep=0.2cm},
        legend cell align={left}
    },
]


\nextgroupplot[
    title={Algorithm Design},
    bar width = 0.15cm,
    nodes near coords,
    nodes near coords style={
        font=\fontsize{5pt}{4pt}\selectfont % This changes the font size to small
    },
    ymax=20,
]
\addplot+[bar shift=0cm, fill=blue!30, draw=blue!80, text=blue!80] coordinates {(A,13)}; \addlegendentry{Zero-shot}
\addplot+[bar shift=0cm, fill=blue!70, draw=blue!100, text=blue!100] coordinates {(B,12)}; \addlegendentry{Zero-shot CoT}
\addplot+[bar shift=0cm, fill=red!30, draw=red!80, text=red!80] coordinates {(C,12)}; \addlegendentry{Few-shot}
\addplot+[bar shift=0cm, fill=red!70, draw=red!100, text=red!100] coordinates {(D,13)}; \addlegendentry{Few-shot CoT}
\addplot+[bar shift=0cm, fill=brown!50, draw=brown!100, text=brown!100] coordinates {(E,13)}; \addlegendentry{Self-debug}
\addplot+[bar shift=0cm, fill=olive, draw=olive, text=olive] coordinates {(F,10)}; \addlegendentry{Self-plan}
\addplot+[bar shift=0cm, fill=violet, draw=violet, text=violet] coordinates {(G,9)}; \addlegendentry{Self-refine}
\addplot+[bar shift=0cm, fill=black!50, draw=black!100, text=black!100] coordinates {(H,15)}; \addlegendentry{Progressive Hint}
\addplot+[bar shift=0cm, fill=teal!50, draw=teal!100, text=teal!100] coordinates {(I,13)}; \addlegendentry{Persona}

\nextgroupplot[
    title={String Manipulation},
    bar width = 0.15cm,
    nodes near coords,
    nodes near coords style={
        font=\fontsize{5pt}{4pt}\selectfont % This changes the font size to small
    },
    ymin=21,
    ymax=40,
]
\addplot+[bar shift=0cm, fill=blue!30, draw=blue!80, text=blue!80] coordinates {(A,34)}; 
\addplot+[bar shift=0cm, fill=blue!70, draw=blue!100, text=blue!100] coordinates {(B,38)}; 
\addplot+[bar shift=0cm, fill=red!30, draw=red!80, text=red!80] coordinates {(C,36)}; 
\addplot+[bar shift=0cm, fill=red!70, draw=red!100, text=red!100] coordinates {(D,40)}; 
\addplot+[bar shift=0cm, fill=brown!50, draw=brown!100, text=brown!100] coordinates {(E,37)}; 
\addplot+[bar shift=0cm, fill=olive, draw=olive, text=olive] coordinates {(F,32)}; 
\addplot+[bar shift=0cm, fill=violet, draw=violet, text=violet] coordinates {(G,21)}; 
\addplot+[bar shift=0cm, fill=black!50, draw=black!100, text=black!100] coordinates {(H,35)}; 
\addplot+[bar shift=0cm, fill=teal!50, draw=teal!100, text=teal!100] coordinates {(I,38)}; 

\nextgroupplot[
    title={List Processing},
    bar width = 0.15cm,
    nodes near coords,
    nodes near coords style={
        font=\fontsize{5pt}{4pt}\selectfont % This changes the font size to small
    },
    ymin=26,
    ymax=46,
]
\addplot+[bar shift=0cm, fill=blue!30, draw=blue!80, text=blue!80] coordinates {(A,43)}; 
\addplot+[bar shift=0cm, fill=blue!70, draw=blue!100, text=blue!100] coordinates {(B,46)}; 
\addplot+[bar shift=0cm, fill=red!30, draw=red!80, text=red!80] coordinates {(C,42)}; 
\addplot+[bar shift=0cm, fill=red!70, draw=red!100, text=red!100] coordinates {(D,43)}; 
\addplot+[bar shift=0cm, fill=brown!50, draw=brown!100, text=brown!100] coordinates {(E,42)}; 
\addplot+[bar shift=0cm, fill=olive, draw=olive, text=olive] coordinates {(F,41)}; 
\addplot+[bar shift=0cm, fill=violet, draw=violet, text=violet] coordinates {(G,26)}; 
\addplot+[bar shift=0cm, fill=black!50, draw=black!100, text=black!100] coordinates {(H,37)}; 
\addplot+[bar shift=0cm, fill=teal!50, draw=teal!100, text=teal!100] coordinates {(I,45)}; 

\nextgroupplot[
    title={Mathematical Computation},
    bar width = 0.15cm,
    nodes near coords,
    nodes near coords style={
        font=\fontsize{5pt}{4pt}\selectfont % This changes the font size to small
    },
    ymin=28,
    ymax=38,
]
\addplot+[bar shift=0cm, fill=blue!30, draw=blue!80, text=blue!80] coordinates {(A,35)}; 
\addplot+[bar shift=0cm, fill=blue!70, draw=blue!100, text=blue!100] coordinates {(B,35)}; 
\addplot+[bar shift=0cm, fill=red!30, draw=red!80, text=red!80] coordinates {(C,34)}; 
\addplot+[bar shift=0cm, fill=red!70, draw=red!100, text=red!100] coordinates {(D,34)}; 
\addplot+[bar shift=0cm, fill=brown!50, draw=brown!100, text=brown!100] coordinates {(E,32)}; 
\addplot+[bar shift=0cm, fill=olive, draw=olive, text=olive] coordinates {(F,32)}; 
\addplot+[bar shift=0cm, fill=violet, draw=violet, text=violet] coordinates {(G,28)}; 
\addplot+[bar shift=0cm, fill=black!50, draw=black!100, text=black!100] coordinates {(H,34)}; 
\addplot+[bar shift=0cm, fill=teal!50, draw=teal!100, text=teal!100] coordinates {(I,34)}; 

\nextgroupplot[
    title={Parsing and Formatting},
    bar width = 0.15cm,
    nodes near coords,
    nodes near coords style={
        font=\fontsize{5pt}{4pt}\selectfont % This changes the font size to small
    },
    ymax=10,
]
\addplot+[bar shift=0cm, fill=blue!30, draw=blue!80, text=blue!80] coordinates {(A,5)}; 
\addplot+[bar shift=0cm, fill=blue!70, draw=blue!100, text=blue!100] coordinates {(B,5)}; 
\addplot+[bar shift=0cm, fill=red!30, draw=red!80, text=red!80] coordinates {(C,5)}; 
\addplot+[bar shift=0cm, fill=red!70, draw=red!100, text=red!100] coordinates {(D,4)}; 
\addplot+[bar shift=0cm, fill=brown!50, draw=brown!100, text=brown!100] coordinates {(E,4)}; 
\addplot+[bar shift=0cm, fill=olive, draw=olive, text=olive] coordinates {(F,4)}; 
\addplot+[bar shift=0cm, fill=violet, draw=violet, text=violet] coordinates {(G,5)}; 
\addplot+[bar shift=0cm, fill=black!50, draw=black!100, text=black!100] coordinates {(H,5)}; 
\addplot+[bar shift=0cm, fill=teal!50, draw=teal!100, text=teal!100] coordinates {(I,5)}; 

\nextgroupplot[
    title={Logical Conditions},
    bar width = 0.15cm,
    nodes near coords,
    nodes near coords style={
        font=\fontsize{5pt}{4pt}\selectfont % This changes the font size to small
    },
    ymax=5,
]
\addplot+[bar shift=0cm, fill=blue!30, draw=blue!80, text=blue!80] coordinates {(A,1)}; 
\addplot+[bar shift=0cm, fill=blue!70, draw=blue!100, text=blue!100] coordinates {(B,1)}; 
\addplot+[bar shift=0cm, fill=red!30, draw=red!80, text=red!80] coordinates {(C,2)}; 
\addplot+[bar shift=0cm, fill=red!70, draw=red!100, text=red!100] coordinates {(D,2)}; 
\addplot+[bar shift=0cm, fill=brown!50, draw=brown!100, text=brown!100] coordinates {(E,1)}; 
\addplot+[bar shift=0cm, fill=olive, draw=olive, text=olive] coordinates {(F,1)}; 
\addplot+[bar shift=0cm, fill=violet, draw=violet, text=violet] coordinates {(G,1)}; 
\addplot+[bar shift=0cm, fill=black!50, draw=black!100, text=black!100] coordinates {(H,1)}; 
\addplot+[bar shift=0cm, fill=teal!50, draw=teal!100, text=teal!100] coordinates {(I,1)}; 




\end{groupplot}

    
\end{tikzpicture}
\caption{The distribution of correct instances across nine PETs
%prompting techniques 
on the HumanEval dataset using GPT-4o.}
\label{HumanEval_distribution}
\end{figure}


==> figs/bar.tex <==
\begin{figure}[ht]
    \centering
    % First bar plot (Pass@1 by Evaluation Steps)
    \begin{adjustbox}{minipage=\linewidth,scale=0.85}
        \begin{tikzpicture}
        \begin{axis}[
            width=0.32\linewidth,
            height=0.4\textheight,
            ybar,
            ylabel={Pass@1},
            symbolic x coords={Evaluation, Inference, Model Construction, Pre-Post Processing, Training},
            xtick=data,
            xticklabel style={rotate=90, anchor=east},
            bar width=15pt,
            nodes near coords,
            title={Pass@1 by Evaluation Steps},
            ymin=0, ymax=0.6,
            major grid style={dashed},
            grid=major,
            legend pos=north west
        ]
        \addplot coordinates {(Evaluation, 0.33) (Inference, 0.34) (Model Construction, 0.26) (Pre-Post Processing, 0.40) (Training, 0.35)};
        \draw[dashed, red] ({rel axis cs:0,0.34}) -- ({rel axis cs:1,0.34}) node[pos=1,above right] {0.34};
        \end{axis}
        \end{tikzpicture}
    \end{adjustbox}
    
    \hfill
    
    % Second bar plot (Pass@1 by Data Types)
    \begin{adjustbox}{minipage=\linewidth,scale=0.85}
        \begin{tikzpicture}
        \begin{axis}[
            width=0.32\linewidth,
            height=0.4\textheight,
            ybar,
            symbolic x coords={Image, Text, Tabled or Structured Array},
            xtick=data,
            xticklabel style={rotate=90, anchor=east},
            bar width=15pt,
            nodes near coords,
            title={Pass@1 by Data Types},
            ymin=0, ymax=0.6,
            major grid style={dashed},
            grid=major,
            legend pos=north west
        ]
        \addplot coordinates {(Image, 0.32) (Text, 0.32) (Tabled or Structured Array, 0.33)};
        \draw[dashed, red] ({rel axis cs:0,0.34}) -- ({rel axis cs:1,0.34}) node[pos=1,above right] {0.34};
        \end{axis}
        \end{tikzpicture}
    \end{adjustbox}
    
    \hfill
    
    % Third bar plot (Pass@1 by Task Types)
    \begin{adjustbox}{minipage=\linewidth,scale=0.85}
        \begin{tikzpicture}
        \begin{axis}[
            width=0.32\linewidth,
            height=0.4\textheight,
            ybar,
            symbolic x coords={Classification, Regression, Recommendation, Prediction, Detection, Segmentation},
            xtick=data,
            xticklabel style={rotate=90, anchor=east},
            bar width=15pt,
            nodes near coords,
            title={Pass@1 by Task Types},
            ymin=0, ymax=0.6,
            major grid style={dashed},
            grid=major,
            legend pos=north west
        ]
        \addplot coordinates {(Classification, 0.31) (Regression, 0.35) (Recommendation, 0.52) (Prediction, 0.32) (Detection, 0.22) (Segmentation, 0.30)};
        \draw[dashed, red] ({rel axis cs:0,0.34}) -- ({rel axis cs:1,0.34}) node[pos=1,above right] {0.34};
        \end{axis}
        \end{tikzpicture}
    \end{adjustbox}
    \label{fig:bar}
    \vspace{-10pt}

\end{figure}

==> figs/distribution.tex <==

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{pics/stats.png}
    \vspace{-7pt}
    \caption{Distribution of the data based on steps in the pipeline
    }
    
    \label{fig:distribution}
    \vspace{-10pt}
    
\end{figure}


==> figs/gray_rgb.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figs/rgb_to.pdf}
    % \vspace{-7pt}
    \caption{An Example of difference variance of Image as data.
    }
    \label{fig:gray_rgb}
    \vspace{-10pt}
\end{figure}

==> figs/image_example.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.6\linewidth]{figs/bounding_margin.pdf}
    % \vspace{-7pt}
    \caption{An example of Image data type}
    \label{fig:image_example}
    \vspace{-10pt}
\end{figure}

==> figs/metrics.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{pics/eval_example.pdf}
    \vspace{-7pt}
    \caption{An example prompt 
    for metrics
    }
    \label{fig:metrics}
    \vspace{-10pt}
\end{figure}

==> figs/recommendation_example.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{pics/recommendation_example.pdf}
    \vspace{-7pt}
    \caption{An Example of data related to recommendation tasks.Gibbs Sampling is a Markov Chain Monte Carlo (MCMC) method used to approximate the joint distribution of variables in a probabilistic model.Gibbs sampling can generate labels for unseen user-item pairs by sampling from the learned distribution, thereby facilitating personalized recommendations.
    }
    \label{fig:recommendation_example}
    \vspace{-10pt}
\end{figure}

==> figs/rejected1.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figs/forward_f.pdf}
    %\vspace{-1pt}
    \caption{An example that GPT is failed to generate the code
    }
    \label{fig:rejected1}
    %\vspace{-10pt}
\end{figure}

==> figs/rejected2.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth, ]{figs/cauchy_last.pdf}
    %\vspace{-7pt}
    \caption{Model Construction example
    }

    \label{fig:rejected2}
    %\vspace{-10pt}
\end{figure}

==> figs/segmentation.tex <==
\vspace{-2pt}
\begin{figure}
    
    \centering
    \includegraphics[width=1\linewidth]{figs/c_transform.pdf}
    \vspace{-7pt}
    \caption{Segmentation Task which GPT-4o failed.
    }
    \label{fig:segmentation}
    \vspace{-10pt}
\end{figure}

==> figs/stats_pie.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=\linewidth]{pics/stats.png}
    \vspace{-7pt}
    \caption{Statistics of DLEval. This figure shows the distribution of data we gather in our benchmark.
    \hung{Can we separate these into three subfigures? put three separate sub label}
    }
    \label{fig:stats}
    \vspace{-10pt}
\end{figure*}

==> figs/text_accept.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figs/ngram_g.pdf}
    \vspace{-7pt}
    \caption{Text data example: Defining n-gram extraction of a list of tokenized text
    %An example of data GPT is able to generate the code for Text related function
    }
    \label{fig:text_accept}
    \vspace{-10pt}
\end{figure}

==> figs/text_example.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.6\linewidth]{figs/margin_tokenize.drawio.pdf}
    \vspace{-7pt}
    \caption{An example prompt for Text data type}
    \label{fig:text_example}
    \vspace{-10pt}
\end{figure}

==> figs/training.tex <==


\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{pics/train_example.pdf}
    \vspace{-7pt}
    \caption{An example prompt 
    for Training
    }
    \label{fig:training}
    \vspace{-10pt}
\end{figure}

==> macros.tex <==

\makeatletter
\newcommand{\mybox}[1]{%
	\setbox0=\hbox{#1}%
	\setlength{\@tempdima}{\dimexpr\wd0+13pt}%
	\begin{tcolorbox}[boxrule=0.5pt, colback=white, arc=4pt,
		left=6pt,right=6pt,top=6pt,bottom=6pt,boxsep=0pt]
		#1
	\end{tcolorbox}
}

%
\newcommand{\tikzcircle}[2][red,fill=red]{\tikz[baseline=-0.5ex]\draw[#1,radius=#2] (0,0) circle ;}%

\definecolor{songcolor}{RGB}{191,191,191}
\newcommand{\todoc}[2]{{\textcolor{#1}{\textbf{#2}}}}
% todo commands:
\newcommand{\todored}[1]{\todoc{red}{\textbf{[[#1]]}}}
\newcommand{\todogreen}[1]{\todoc{green}{\textbf{[[#1]]}}}
\newcommand{\todoblue}[1]{\todoc{blue}{\textbf{[[#1]]}}}
\newcommand{\todogray}[1]{\todoc{Gray}{\textbf{[[#1]]}}}
\newcommand{\todoorange}[1]{\todoc{orange}{\textbf{[[#1]]}}}
\newcommand{\todobrown}[1]{\todoc{brown}{\textbf{[[#1]]}}}
\newcommand{\todopurple}[1]{\todoc{purple}{\textbf{[[#1]]}}}
\newcommand{\todoamber}[1]{\todoc{teal}{\textbf{[[#1]]}}}
%
%\newcommand{\tikzcircle}[2][red,fill=red]{\tikz[baseline=-0.5ex]\draw[#1,radius=#2] (0,0) circle ;}%


\newcommand{\add}[1]{\todoc{blue}{#1}}
\newcommand{\hung}[1]{\todogreen{Hung: #1}}
\newcommand{\john}[1]{\todoorange{John: #1}}
\newcommand{\alireza}[1]{\todopurple{Alireza: #1}}





\newcommand{\review}[1]{{\textit{#1}}~\\}
\newcommand{\respto}[1]{
\fcolorbox{black}{black!15}{
\label{response:#1}
\bf
  \scriptsize Review {#1}}~
}
\newcommand{\citerespexp}[1]{
\fcolorbox{black}{black!15}{
 \bf
  \scriptsize Review {#1}}~{\bf{on page \pageref{response:#1}}}
}

\newcommand{\citeresp}[1]{
\fcolorbox{black}{black!15}{
 \bf
  \scriptsize Review {#1}}
}


% --- for revision
\newcommand{\rev}[1]{\textcolor{purple}{\st{#1}}}
%\newcommand{\rev}[1]{}
%\newcommand{\add}[1]{\textcolor{blue}{{#1}}

%% space in some tables.  BUT have it here, such that you can always renew it
\newcommand{\ts}{$\;$}
\newcommand{\tS}{$\;$}
\newcommand{\tts}{\ \ \ \ \ }
\newcommand{\tss}{\ \ \ $\;$}
\newcommand{\ttts}{$\;$}
\newcommand{\decentHLine}{\noalign{\hrule height 1.04pt}}



==> tabs/Datatype.tex <==
\begin{table}[h]
    \centering
    \caption{Count of different Data category}
    \label{tab:data_type}
    \resizebox{\linewidth}{!}{ % Adjust the table to the width of the document
    \begin{tabular}{c c c c c } % Bold header and centered columns
    
        \toprule
        \textbf{Data Type} & \textbf{Image} & \textbf{Text} & \textbf{Structured Data} & \textbf{Not Obvious Input Type}            \\
        \hline
        \textbf{Counts} & 238 & 28 & 84 & 168 \\
        % \hline
        \bottomrule
    \end{tabular}
   }
    
    
\end{table}

==> tabs/Tasks.tex <==
\begin{table}[h]
    \centering
     \caption{Count of different tasks category}
    \label{tab:tasks}
    \resizebox{\linewidth}{!}{ % Adjust the table to the width of the document
    \begin{tabular}{c c c c c c c c } % Bold header and centered columns
    
        \toprule
        \textbf{Task Type} & \textbf{Classification} & \textbf{Regression} & \textbf{Recommendation} & \textbf{Prediction} & \textbf{Detection} & \textbf{Segmentation} & \textbf{Common Tasks} \\
        \midrule
        Count & 60 & 14 & 17 & 24 & 37 & 40 & 328 \\
        \bottomrule
    \end{tabular}
    }
    
   
\end{table}

==> tabs/Taxonomy_prev1.tex <==
\begin{table}[h!]
\centering
     \caption{Distribution of bugs in general LLM code based on Tambon et. al\cite{tambon2024bugs}}
    \label{tab:general_bug}
   
\begin{tabular}{ll}
Bug Type                      & Occurrence(\%) \\ \hline
Generated code deviates from prompt intention             & 20.77          \\
Missing parenthesis, semicolon, or other syntax issues                   & 6.11           \\
Redundant conditions, unnecessary casting                 & 9.57           \\
Code overly relies on examples from the prompt           & 6.52           \\
Incorrect input type in function calls & 5.91           \\
Fails to handle edge cases          & 15.27          \\
Uses nonexistent or undefined object          & 9.57           \\
Incorrect/nonexistent attributes for objects or modules               & 8.55           \\
Incomplete Generation         & 9.57           \\
Adds non-requested features to code   & 8.15          
\end{tabular}
\end{table}

==> tabs/Taxonomy_prev2.tex <==
\begin{table}[h!]
\centering
     \caption{Distribution of bugs in Deep Learning code based on ~\cite{islam2019comprehensive}}
    \label{tab:dl_bug}
\begin{tabular}{lll}
Bug Category             & Github & StackOverflow \\ \hline
API Bug                  & 272    & 44            \\
Data Bug                 & 54     & 110           \\
Control and Sequence Bug & 14     & 16            \\
Initialization Bug       & 15     & 23            \\
Dataflow Bug             & 105    & 48            \\
Logic Bug                & 61     & 141           \\
Processing Bug           & 35     & 32           
\end{tabular}
\end{table}

==> tabs/statistics.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[]
\caption{Statistics of DLEval}
\label{tabs:statistics}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}cccccccc@{}}
\multirow{2}{*}{\textbf{Stage In Pipeline}} &
  Pre-Post Processing &
  \multicolumn{2}{c}{Model Construction} &
  Training &
  Inference &
  \multicolumn{2}{c}{Evaluation} \\ \cmidrule(l){2-8} 
 & 210     & \multicolumn{2}{c}{119}        & 75    & 58     & \multicolumn{2}{c}{58}     \\
\\
\multirow{2}{*}{\textbf{Data Types}} &
  \multicolumn{2}{c}{Image} &
  \multicolumn{2}{c}{Text} &
  \multicolumn{2}{c}{Structured array} &
  Others \\ \cmidrule(l){2-8} 
 & \multicolumn{2}{c}{238} & \multicolumn{2}{c}{28} & \multicolumn{2}{c}{84} & 168        \\
\\
\multirow{2}{*}{\textbf{Task Type}} &
  Classification &
  Regression &
  Detection &
  Segmentation &
  Recommendation &
  Prediction &
  General Tasks \\ \cmidrule(l){2-8} 
 & 60      & 14            & 37             & 40    & 17     & 24            & 328       
\end{tabular}
}
\end{table*}
